Iterative Pre-Conditioning for Expediting the Gradient-Descent Method: The Distributed Linear Least-Squares Problem

This paper considers the multi-agent linear least-squares problem in a server-agent network. In this problem, the system comprises multiple agents, each having a set of local data points, that are connected to a server. The goal for the agents is to compute a linear mathematical model that optimally fits the collective data points held by all the agents, without sharing their individual local data points. This goal can be achieved, in principle, using the server-agent variant of the traditional iterative gradient-descent method. The gradient-descent method converges linearly to a solution, and its rate of convergence is lower bounded by the conditioning of the agents' collective data points. If the data points are ill-conditioned, the gradient-descent method may require a large number of iterations to converge. We propose an iterative pre-conditioning technique that mitigates the deleterious effect of the conditioning of data points on the rate of convergence of the gradient-descent method. We rigorously show that the resulting pre-conditioned gradient-descent method, with the proposed iterative pre-conditioning, achieves superlinear convergence when the least-squares problem has a unique solution. In general, the convergence is linear with improved rate of convergence in comparison to the traditional gradient-descent method and the state-of-the-art accelerated gradient-descent methods. We further illustrate the improved rate of convergence of our proposed algorithm through experiments on different real-world least-squares problems in both noise-free and noisy computation environment.

==> analysis.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{CONVERGENCE ANALYSIS}
\label{sec:analysis}

In this section, we present a convergence analysis of our proposed algorithm in Section~\ref{sec:algo}. At first, we consider the case where the distributed least-squares problem~\eqref{eqn:opt_1} has more than one solutions. We establish linear convergence in this case. Next, we consider unique solution $x^*$ of~\eqref{eqn:opt_1} and establish superlinear convergence of Algorithm~\ref{algo_1}.  We limit the analysis in this section to deterministic case and defer the analysis under system noise to Section~\ref{sec:noise}.\\

\subsection{Linear Convergence}

The results presented in this subsection hold for the general tall matrix $A$. To be able to present the convergence of Algorithm~\ref{algo_1}, we introduce the following notations.
\begin{itemize}
\setlength\itemsep{0.5em}
    \item Let, \[K^*_{\beta} = \left(\A+\beta I\right)^{-1}.\] Note that, the matrix $A^T A$ is positive semi-definite. Thus, $\left(\A+\beta I\right)$ is positive definite for $\beta > 0$. So, $\left(\A+\beta I\right)$ is invertible and $K^*_{\beta}$ is well-defined.
    \item Let $k_j^*$ be the $j$-th column of $K^*_{\beta}$, $j=1,\ldots,d$.
    \item  Let, $\lambda$ and $\gamma$ denote the smallest and largest eigenvalue of $\A$, respectively.
    \item Let $\gamma_r$ denote the smallest non-zero eigenvalue of $\A$.
    \item For a matrix $M \in \R^{m \times n}$, let $\norm{M}_F$ denote its Frobenius norm, which is defined as the square root of the sum of squares of its elements,
$\norm{M}_F := \sqrt{\sum_{i=1}^m \sum_{j=1}^n m_{ij}^2}$~\cite{meyer2000matrix}. The Frobenius norm can also be written as the square root of the sum of squares of the $2$-norm of its columns.
    \item Let $x^*$ be a point of minima of~\eqref{eqn:opt_1} and $x(t)$ be the estimate at iteration $t$ of Algorithm~\ref{algo_1}. Define the estimation error for iteration $t$ as
\begin{align}
    z(t) := x(t) - x^*. \label{eqn:err}
\end{align}
\printcomment{ +++ as $x^*$ is not unique, we should define $z(t) = x(t) - [x(t)]_{X^*}$ where $[x(t)]_{X^*}$ denotes the projection of $x(t)$ onto $X^*$. Note as $X^*$ is closed and convex $[x(t)]_{X^*}$ exists and is unique for all $t$ +++ }

    \item For a matrix $M$, let its kernel and the subspace orthogonal to it be denoted by $\mathcal{N}(M)$ and $\mathcal{N}(M)^{\perp}$, respectively. 
    \item Let,
    \begin{align}
        \rho^*_K := \frac{\lambda - \gamma }{\lambda + \gamma +2\beta}, \, \ro := \dfrac{(\lambda - \gamma_r)\beta }{(\lambda + \gamma_r)\beta + 2\lambda \gamma_r}, \, \sigma_0 := \delta \lambda \norm{K(-1)-K^*_{\beta}}_F. \label{eqn:rho_def}
    \end{align}
\end{itemize}

% ============================================================================= %
% ============================================================================= %
\begin{comment}
\begin{figure}[thpb]  
\centering
\begin{tikzpicture}
\shade[left color=blue!20,right color=red!20] (0,0) -- (4,0) -- (6,2) -- (2,2) -- (0,0);
\draw [thick, color=black] (1,0.3) node {$\mathcal{N}(A)$};
\coordinate[label=above:$x(t)$] (A) at (4.5,3);
\coordinate[label=left:$x^*$] (B) at (2,1);
\coordinate[] (C) at (4.5,1);
\draw [thick,color=purple] (A) -- (C) -- (B) -- (A);
\draw (3.4,2.5) node {$z(t)$};
\draw (5,2.5) node {$z(t)^{\perp}$};
\end{tikzpicture}
\caption{Schematic illustration for $z(t)$ and $z(t)^{\perp}$.}
\label{fig:zperp}
\end{figure}
\end{comment}
% ============================================================================= %
% ============================================================================= %

Since any point of minima $x^*$ satisfies $\A x^* = A^T b $, we have $\A\left(x^*+y\right) = \A x^*+\A y = A^T b$ if $y \in \mathcal{N}(\A)$. Thus, $\left(x^*+y\right)$ is also a point of minima of~\eqref{eqn:opt_1} for $y \in \mathcal{N}(\A)$. So, $x(t)$ converges to a solution if $z(t)$ converges to the kernel of $\A$. Hence, we would want to reduce the distance between $z(t)$ and kernel of $\A$ as the iterations proceed. The distance between $z(t)$ and kernel of $\A$ is given by $\norm{z(t)^{\perp}}$, where $z(t)^{\perp}$ is the component of the vector $z(t)$ orthogonal to the kernel of $\A$. The following theorem shows convergence of $z(t)^{\perp}$ to the zero vector at a linear time-varying rate, thereby establishing linear convergence of Algorithm~\ref{algo_1} to a point of minima. \\

\noindent \fbox{\begin{minipage}{\textwidth}
\begin{theorem} \label{thm:thm1}
Consider Algorithm 1 with $\beta > 0$. Then, for arbitrary $x(0)$ and $K(-1)$:
\begin{itemize}
    \item There exists $\delta > 0$ for which there is a positive value $\rho_{\beta} < 1$ such that
\begin{align}
    \norm{z(t+1)^{\perp}} \leq \left(\rho_{\beta}+\sigma_0 (\rho^*_K)^{t+1}\right) \norm{z(t)^{\perp}}, \, \forall t, \label{eqn:zperp_6}
\end{align}
where $\rho_{\beta} \geq \ro$.
    \item $\underset{t \rightarrow \infty}{lim} \, z(t)^{\perp} = 0$.
    \item $x(t)$ converges to a solution of~\eqref{eqn:opt_1} as $t \rightarrow \infty$.
\end{itemize}
\end{theorem}
\end{minipage}}
~\\

Proof of Theorem~\ref{thm:thm1} is deferred to Appendix~\ref{prf:thm1}.\\

\begin{remarks}
It is desirable to have as small rate of convergence as possible. The smallest rate of convergence in~\eqref{eqn:zperp_6} depends on $\rho_K^*$ as well as $\ro$. Since $\dfrac{d \rho_K^*}{d \beta} < 0$ and $\dfrac{d \ro}{d \beta} > 0$, there exists a trade-off for $\beta$ between $\rho_K^*$ and $\ro$. 
\end{remarks}

Theorem~\ref{thm:thm1} tells us that Algorithm~\ref{algo_1} converges at a linear rate of $\left(\rho_{\beta}+\sigma_0 (\rho^*_K)^{t+1}\right)$. We present another result that essentially compares the convergence rate of our algorithm with Distributed Gradient Descent (DGD), Distributed Nesterov's Accelerated Gradient Descent (D-NAG) and Distributed Heavy Ball (D-HBM) methods. These methods are popular distributed gradient-based, and they are known to have a linear rate of convergence. Besides, the same result helps us experimentally comparing with the Accelerated Projection-based Consensus (APC) method, which has been speculated to have the fastest rate of convergence among the existing distributed gradient methods. \\

We define a few notations necessary for the subsequent analysis.
\begin{itemize}
\setlength\itemsep{0.5em}
    \item Let $\rho_{GD}$, $\rho_{NAG}$ and $\rho_{HBM}$ respectively denote the smallest convergence rate of DGD, D-NAG and D-HBM method. We use an index `$a$' taking the values $\{1,2,3\}$, for referring to each of these three algorithms respectively, and their smallest convergence rates are referred to as $\rho^{(a)}, \, a=1,2,3$. It is known that~\cite{azizan2019distributed},
    \begin{align}
        \rho_{NAG} & = 1 - \dfrac{2}{\sqrt{3\kappa(\A)+1}}, \label{eqn:rho_nag} \\
        \rho_{HBM} & = \dfrac{\sqrt{\kappa(\A)-1}}{\sqrt{\kappa(\A)-1}}. \label{eqn:rho_hbm}
    \end{align}
    \item For a positive number $x$, let $\floor{x}$ denote the largest integer less than or equal to $x$.
    \item Let,
    \begin{align}
        \tau^{(a)} & := \floor{\dfrac{log \left(\dfrac{\sigma_0}{\rho^{(a)} - \ro} \right)}{log \left(\dfrac{1}{\rho_K^*} \right)}}, \label{eqn:tau_a}\\
        r^{(a)} & := \dfrac{\left(\ro+\sigma_0 (\rho^*_K)^{\tau^{(a)}+2}\right)}{\rho^{(a)}}, \label{eqn:r_a}\\
        c^{(a)} & := \left( \dfrac{\ro+\sigma_0 \rho^*_K}{r^{(a)} \, \rho^{(a)}} \right)^{\tau^{(a)} + 1}, \label{eqn:c_a}\\
        t^{(a)} & := \floor{\dfrac{log \left(c^{(a)} \right)}{log \left(\dfrac{1}{r^{a)}} \right)}}. \label{eqn:tsw_a}
    \end{align}
\end{itemize}

Recall that, $\norm{z(t)^{\perp}}$ measures the distance between the current estimate $x(t)$ and a desired point of minima $x^*$. The following lemma formally compares the known theoretical upper bound of the distance $\norm{z(t)^{\perp}}$ for DGD, D-NAG, and D-HBM with Algorithm~\ref{algo_1}. 
Note that, $\kappa(\A) = 1$ is the trivial case where $\rho_{GD} = 0$ and the DGD algorithm converges after just one iteration. We present the result for the non-trivial $\kappa(\A)>1$. \\

\noindent \fbox{\begin{minipage}{\textwidth}
\begin{lemma} \label{thm:lem1}
Consider Algorithm~\ref{algo_1} and assume $\kappa(\A) > 1$. If $a=1$, then for $\beta > 0$ we have,
\begin{itemize}
    \item $r^{(a)} < 1$ and
\begin{align}
    \norm{z(t+1)^{\perp}} \leq c^{(a)} \left(r^{(a)} \, \rho^{(a)} \right)^{t+1} \, \norm{z(0)^{\perp}}, \, \forall t > \tau \label{eqn:z2_lem1}
\end{align}
    \item We have
    \begin{align}
    c^{(a)} \left(r^{(a)} \, \rho^{(a)} \right)^{t+1} < \left(\rho^{(a)}\right)^{t+1}, \, \forall t > t^{(a)}. \label{eqn:tsw_lem1}
\end{align}
\end{itemize}
If $a=2$, then~\eqref{eqn:z2_lem1} and~\eqref{eqn:tsw_lem1} hold for $\beta < \sqrt{3\lambda \gamma_r}$. If $a=3$, then~\eqref{eqn:z2_lem1} and~\eqref{eqn:tsw_lem1} hold for $\beta < \sqrt{\lambda \gamma_r}$.
\end{lemma}
\end{minipage}}
~\\

%Proof of Lemma~\ref{thm:lem1} is deferred to Appendix~\ref{prf:lem1}.\\

\begin{remarks}
Lemma~\ref{thm:lem1} tells us that, even though Algorithm~\ref{algo_1} might be initially slower than the DGD, D-NAG or D-HBM algorithm, after a finite number of iterations $t^{(a)}$ Algorithm~\ref{algo_1} is guaranteed to have smaller error bound compared to any of them with identical initialization $x(0)$ and arbitrary $K(-1)$. More importantly, this error bound of Algorithm-I decreases $r^{(a)}$-exponentially faster compared to any of those three algorithms. The point $t^{(a)}$ in the iterations essentially depends on the convergence rates of Algorithm~\ref{algo_1} and the algorithm with whom it is compared. Moreover, Lemma~\ref{thm:lem1} also provides a constructive way for evaluating $t^{(a)}$. Note that $t^{(a)}$ is a sufficient iteration index, after which Algorithm~\ref{algo_1} is guaranteed to be faster than the other algorithm. The actual index could be smaller than $t^{(a)}$.
Gradient-based methods are known to suffer from slower convergence when the algorithm gets closer to a minimum, especially if the condition number $\kappa(\A)$ is large. Thus, Algorithm~\ref{algo_1} is useful in mitigating that effect, as we will demonstrate via simulations in Section~\ref{sec:exp}. Note that, using Lemma~\ref{thm:lem1} we can formally compare Algorithm~\ref{algo_1} with any other algorithm compared to which Algorithm~\ref{algo_1} has a smaller rate of convergence after a finite time.
%This will be demonstrated in the experiments where we will use Lemma~\ref{thm:lem1} to compare with APC as well.
\end{remarks}

\printcomment{ +++ Isn't the case of unique solution a special case of the above ? ++++}

\subsection{Superlinear Convergence}

In this subsection, we consider the optimization problem~\eqref{eqn:opt_1} when the matrix $\A$ is positive definite. In this case, $\mathcal{N}(A) = \{\theta\}$ which means~\eqref{eqn:opt_1} has a unique solution $x^*$ and $z(t) = z(t)^{\perp}$. Also, $\gamma > 0$ and $\gamma_r = \gamma$. Here, $\theta$ denotes the zero vector in $\R^n$. When $\A$ is positive definite, Algorithm~\ref{algo_1} with $\beta = 0$ converges to $x^*$ at a superlinear rate. The next theorem formally proves this claim. \\

\noindent \textbf{Assumption 1}: Assume that the matrix $A$ is full rank. 

This assumption necessarily means that, $\A$ is a positive definite matrix, and the minimization problem~\eqref{eqn:opt_1} has a unique solution $x^*$. \\ 

\noindent \fbox{\begin{minipage}{\textwidth}
\begin{theorem} \label{thm:thm2}
Consider Algorithm 1 with $\beta = 0$. Under Assumption 1, for arbitrary $x(0)$ and $K(-1)$:
\begin{itemize}
    \item There exists $\delta > 0$ for which there is a positive value $\rho_{\beta} < 1$ such that
\begin{align}
    \norm{z(t+1)} \leq \left(\sigma_0 (\rho_{GD})^{t+1}\right) \norm{z(t)}, \, \forall t. \label{eqn:zperp_7}
\end{align}
    \item $\underset{t \rightarrow \infty}{lim} \, \dfrac{\norm{z(t+1)}}{\norm{z(t)}} = 0$.
\end{itemize}
\end{theorem}
\end{minipage}}
~\\

\begin{proof}
Under Assumption 1, $\A$ is positive definite and $\left(\A\right)^{-1}$ is defined. Assumption 1 also implies that $\mathcal{N}(A) = \{\theta\}$ and $z(t) = z(t)^{\perp}$. Note that, $\rho_K^* = \rho_{GD}$ and $\ro = 0$ when $\beta = 0$. As Theorem~\ref{thm:thm1} holds true for $K^*_{\beta} = K^*_0$ and $\beta = 0$, from~\eqref{eqn:zperp_6} we obtain~\eqref{eqn:zperp_7}.

From~\eqref{eqn:zperp_7},
\begin{align*}
    \dfrac{\norm{z(t+1)}}{\norm{z(t)}} \leq \sigma_0 (\rho_{GD})^{t+1}.
\end{align*}
This implies that if $\rho_{GD} < 1$ then
\begin{align*}
    \underset{t \rightarrow \infty}{\lim} \, \dfrac{\norm{z(t+1)}}{\norm{z(t)}} \leq \underset{t \rightarrow \infty}{\lim} \, \sigma_0 (\rho_{GD})^{t+1} = 0.
\end{align*}
\end{proof}

%Proof of Theorem~\ref{thm:thm1} is deferred to Appendix~\ref{prf:thm2}.\\

Theorem~\ref{thm:thm2} tells us that, Algorithm~\ref{algo_1} superlinearly converges to the minima of the distributed least-squares problem ~\eqref{eqn:opt_1} with an unique solution.  It is known that distributed methods like DGD, D-NAG, D-HBM, APC have a linear rate of convergence. Thus, Algorithm~\ref{algo_1} has a superior rate of convergence than these methods, as well as other existing methods with linear convergence. \\












































%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
The results presented in this section hold for general tall matrix $A$. As a special case, if the matrix $\A$ is positive definite, then~\eqref{eqn:opt_1} has a unique solution $x^*$. In this case, $\mathcal{N}(A) = \{\theta\}$ which means $z(t) = z(t)^{\perp}$. Also, $\gamma > 0$ and $\gamma_r = \gamma$. Here, $\theta$ denotes the zero vector in $\R^n$. \\

Proof of Lemma~\ref{thm:lem3} is deferred to Appendix~\ref{prf:lem3}.\\

\begin{remarks}
From~\eqref{eqn:z1}, we have
\[ \norm{z_2(t+1)^{\perp}} \leq \left(\Pi_{k=0}^{t} \, \eta_k\right) \norm{z(0)^{\perp}}, \, \forall t. \] 
This gives us a framework for formal comparison of the convergence rate of two algorithms whose rate of convergence satisfies the conditions in Lemma~\ref{thm:lem3}. If the convergence rate of Algorithm-I is less than that of Algorithm-II after a finite number of iterations $\tau$, even if Algorithm-II is faster than Algorithm-I at the initial stage, then Algorithm-I is guaranteed to have smaller error bound than Algorithm-II after a finite number of iterations $t_{sw}$ and this error bound of Algorithm-I decreases $\Bar{r}$-exponentially faster compared to Algorithm-II. The point $t_{sw}$ in the iterations essentially depends on the convergence rates of those two algorithms. Moreover, if $\tau$ is known then Lemma~\ref{thm:lem3} also provides a constructive way for evaluating $t_{sw}$. Note that $t_{sw}$ is a sufficient iteration index after which Algorithm-I is guaranteed to be faster than Algorithm-II. The actual index could be smaller than $t_{sw}$.
\end{remarks}

Now we present the main result of this section. Recall that, $z(t)^{\perp}$ is the component of estimation error $z(t)$ for iteration $t$ of Algorithm~\ref{algo_1} along the subspace orthogonal to kernel of $A$. \\

\noindent \fbox{\begin{minipage}{\textwidth}
\begin{theorem} \label{thm:thm1}
Consider Algorithm~\ref{algo_1} with $\beta > 0$. Then there exists $\delta > 0$ for which,
\begin{itemize}
    \item There exists $\tau = \floor{\dfrac{log \left(\dfrac{\sigma_0}{\rho_{GD} - \rho_{\beta}} \right)}{log \left(\dfrac{1}{\rho_K^*} \right)}}$ such that
\begin{align}
    \norm{z(t+1)^{\perp}} \leq c \left(r_{\tau+1} \, \rho_{GD} \right)^{t+1} \, \norm{z(0)^{\perp}}, \, \forall t > \tau \label{eqn:z2}
\end{align}
where $r_{\tau+1} := \dfrac{\left(\rho_{\beta}+\sigma_0 (\rho^*_K)^{\tau+2}\right)}{\rho_{GD}} < 1$, and $c := \left( \dfrac{\rho_{\beta}+\sigma_0 \rho^*_K}{r_{\tau+1} \, \rho_{GD}} \right)^{\tau + 1}$ is a constant.
    \item $\underset{t \rightarrow \infty}{lim} \, z(t)^{\perp} = 0$.
    \item There exists $t_{sw} := \floor{\dfrac{log \left(c \right)}{log \left(\dfrac{1}{r_{\tau+1}} \right)}}$ such that
    \begin{align}
    c \left(r_{\tau+1} \, \rho_{GD} \right)^{t+1} < \rho_{GD}^{t+1}, \, \forall t > t_{sw}. \label{eqn:tsw}
\end{align}
\end{itemize}
\end{theorem}
\end{minipage}}
~\\

Proof of Theorem~\ref{thm:thm1} is deferred to Appendix~\ref{prf:thm1}.\\
\end{comment}


\begin{comment}
\noindent \fbox{\begin{minipage}{\textwidth}
\begin{lemma} \label{thm:lem3}
Suppose the least upper-bound of the norm of $z_i(t)^{\perp}, \, i=1,2,$ are as follows:
\begin{align}
    \norm{z_1(t+1)^{\perp}} & \leq \alpha_t \norm{z_1(t)^{\perp}},
    \norm{z_2(t+1)^{\perp}} \leq \eta \norm{z_2(t)^{\perp}}, \, \forall t \label{eqn:z1} 
\end{align}
where $\{\alpha_t > 0\}_{t \geq 0}$ is a strictly decreasing sequence and $0 < \eta  < 1$.
If both the algorithms are identically initialized with $z(0) \in \R^n$, then 
\begin{itemize}
    \item There exists $\tau$ such that
\begin{align}
    \norm{z_1(t+1)^{\perp}} \leq c \left(r_{\tau}\eta \right)^{t+1} \, \norm{z(0)^{\perp}}, \, \forall t > \tau \label{eqn:z2}
\end{align}
where $\tau$ is the least integer satisfying $\alpha_{\tau} < \eta$,
$r_{\tau} := \dfrac{\alpha_{\tau}}{\eta} < 1$, and $c := \left( \dfrac{\alpha_{0}}{r_{\tau} \eta} \right)^{\tau + 1}$ is a constant.
    \item $\underset{t \rightarrow \infty}{lim} \, z_1(t)^{\perp} = 0$.
    \item There exists $t_{sw} := \floor{\dfrac{log \left(\dfrac{1}{c} \right)}{log \left(\dfrac{1}{r_{\tau}} \right)}}$ such that
    \begin{align}
    c \left(r_{\tau}\eta \right)^{t+1} < \eta^{t+1}, \, \forall t > t_{sw}. \label{eqn:tsw}
\end{align}
\end{itemize}
\end{lemma}
\end{minipage}}
~\\
\end{comment}


==> proof_lemma1.tex <==
\subsection{Proof of Lemma~\ref{thm:lem1}}
\label{prf:lem1}

We make a claim that compares the convergence rate of two algorithms for solving~\eqref{eqn:opt_1}, both of them having time-varying rate of contraction, one of which is smaller than the other after a finite number of iterations. We refer these algorithms as Algorithm-I and Algorithm-II. Our result is a direct application of this claim, as will be shown shortly. \\

To present this claim, we define a few notations. 
\begin{itemize}
\setlength\itemsep{0.5em}
    \item Let the estimate of optimum point $x^*$ computed by Algorithm-I and Algorithm-II be denoted by $x_1(t)$ and $x_2(t)$, respectively, after $t$ iterations. 
    Define the estimation errors $z_1(t) := x_1(t)-x^*$ and $z_2(t) := x_2(t)-x^*$.
    \item The least upper-bound of $\norm{z_i(t)^{\perp}}, \, i=1,2,$ are as follows:
\begin{align}
    \norm{z_1(t+1)^{\perp}} & \leq \alpha_t \norm{z_1(t)^{\perp}} \, \text{and} \,
    \norm{z_2(t+1)^{\perp}} \leq \eta_t \norm{z_2(t)^{\perp}}, \, \forall t. \label{eqn:z1} 
\end{align}
    \item Define $r_t := \dfrac{\alpha_t}{\eta_t}$ and $\Bar{r} := \underset{t>\tau}{max} \, r_t$.
    \item Define
    \begin{align}
        c := \left(\dfrac{\alpha_{0}}{\Bar{r}}\right)^{\tau+1} \left(\dfrac{1}{\Pi_{k=0}^{\tau} \, \eta_k}\right), \, 
        t_{sw} := \floor{\dfrac{log \left(c \right)}{log \left(\dfrac{1}{\Bar{r}} \right)}}.
    \end{align}
\end{itemize}


\noindent \fbox{\begin{minipage}{\textwidth}
\begin{claim} \label{thm:clm3}
Suppose $\{\alpha_t > 0\}_{t \geq 0}$ is a strictly decreasing sequence such that $\alpha_t < \eta_t < 1 \, \forall t>\tau$. 
If both the algorithms are identically initialized with $x(0) \in \R^n$, then 
\begin{itemize}
    \item $\Bar{r} < 1$ and
\begin{align}
    \norm{z_1(t+1)^{\perp}} \leq c \left(\Bar{r}\right)^{t+1} \, \left(\Pi_{k=0}^{t} \, \eta_k\right) \, \norm{z(0)^{\perp}}, \, \forall t > \tau \label{eqn:z2}
\end{align}
    \item We have
    \begin{align}
    c \left(\Bar{r}\right)^{t+1} \, \left(\Pi_{k=0}^{t} \, \eta_k\right) < \left(\Pi_{k=0}^{t} \, \eta_k\right), \, \forall t > t_{sw}. \label{eqn:tsw}
\end{align}
\end{itemize}
\end{claim}
\end{minipage}}
~\\

\begin{proof}
From~\eqref{eqn:z1}, we get
\begin{align}
    & \norm{z_1(t+1)^{\perp}} \leq \left(\Pi_{k=\tau+1}^t \, \alpha_k\right) \norm{z_1(\tau + 1)^{\perp}}, \, \forall t > \tau. \label{eqn:z3}
\end{align}
From~\eqref{eqn:z1} and the fact that $\{\alpha_t > 0\}_{t \geq 0}$ is a strictly decreasing sequence, we have
\begin{align}
    & \norm{z_1(\tau+1)^{\perp}} \leq \alpha_{\tau} \norm{z_1(\tau)^{\perp}} \leq \alpha_{0} \norm{z_1(\tau)^{\perp}}, \nonumber \\
    \implies & \norm{z_1(\tau+1)^{\perp}} \leq \alpha_{0}^{\tau+1} \norm{z(0)^{\perp}}. \label{eqn:z4}
\end{align}
Combining~\eqref{eqn:z3} and~\eqref{eqn:z4},
\begin{align*}
    \norm{z_1(t+1)^{\perp}} & \leq \left(\Pi_{k=\tau+1}^t \, \alpha_k\right) \alpha_{0}^{\tau+1} \norm{z(0)^{\perp}} \\
    & = \left(\Pi_{k=\tau+1}^t \, r_k \eta_k\right) \alpha_{0}^{\tau+1} \norm{z(0)^{\perp}} \\
    & = \left(\Pi_{k=\tau+1}^t \, r_k \eta_k\right) \left(\Pi_{k=0}^{\tau} \, \eta_k\right) \left(\dfrac{\alpha_{0}^{\tau+1}}{\Pi_{k=0}^{\tau} \, \eta_k}\right) \norm{z(0)^{\perp}} \\
    & \leq \left(\Pi_{k=\tau+1}^t \, \Bar{r} \eta_k\right) \left(\Pi_{k=0}^{\tau} \, \eta_k\right) \left(\dfrac{\alpha_{0}^{\tau+1}}{\Pi_{k=0}^{\tau} \, \eta_k}\right) \norm{z(0)^{\perp}} \\
    & = \left(\Bar{r}\right)^{t-\tau} \left(\Pi_{k=0}^{t} \, \eta_k\right) \left(\dfrac{\alpha_{0}^{\tau+1}}{\Pi_{k=0}^{\tau} \, \eta_k}\right) \norm{z(0)^{\perp}} \\
    & = \left(\Bar{r}\right)^{t+1} \left(\Pi_{k=0}^{t} \, \eta_k\right) \, \underbrace{\left(\dfrac{\alpha_{0}}{\Bar{r}}\right)^{\tau+1} \left(\dfrac{1}{\Pi_{k=0}^{\tau} \, \eta_k}\right)}_c \, \norm{z(0)^{\perp}}, \, \forall t>\tau.
\end{align*}
Since $\alpha_t < \eta_t < 1 \, \forall t>\tau$, we have $r_t = \dfrac{\alpha_t}{\eta_t} < 1 \, \forall t>\tau$. Thus, $\Bar{r} := \underset{t>\tau}{max} \, r_t < 1$. This proves the first part of the claim.

%Since both $\Bar{r}, \, \eta_t \in (0,1)  \, \forall t>\tau$, we have $\underset{t \rightarrow \infty}{\lim} \, \left(\Bar{r}\right)^{t+1} \, \left(\Pi_{k=0}^{t} \, \eta_k\right) = 0$, and the second part of the clam follows from~\eqref{eqn:z2}.

Since $\Bar{r}< 1$, there exists $t_{sw} < \infty$ such that~\eqref{eqn:tsw} holds. To find an explicit form of $t_{sw}$, we want
\begin{align*}
    & c \left(\Bar{r}\right)^{t+1} \, \left(\Pi_{k=0}^{t} \, \eta_k\right) < \left(\Pi_{k=0}^{t} \, \eta_k\right) \\
    \iff & c \, \left(\Bar{r}\right)^{t+1} < 1 \\
    \iff & \left(\dfrac{1}{\Bar{r}} \right)^{t+1} > c \\
    \iff & t > \dfrac{log \left(c \right)}{log \left(\dfrac{1}{\Bar{r}} \right)} - 1.
\end{align*}
Hence, the least such integer $t_{sw}$ is given by $\floor{\dfrac{log \left(c \right)}{log \left(\dfrac{1}{\Bar{r}} \right)}}$, and the second part of the claim follows.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
Since $\{\alpha_t > 0\}_{t \geq 0}$ is a strictly decreasing sequence and $0< \eta < 1$ is a constant, there exists a positive integer $\tau$ such that $\alpha_t < \eta \, \forall t > \tau$. Then, $r_{\tau} := \dfrac{\alpha_{t}}{\eta} < 1$.

From~\eqref{eqn:z1} and the fact that $\{\alpha_t > 0\}_{t \geq 0}$ is a strictly decreasing sequence, we get
\begin{align}
    & \norm{z_1(t+1)^{\perp}} \leq \alpha_{\tau} \norm{z_1(t)^{\perp}}, \, \forall t > \tau \nonumber \\
    \implies & \norm{z_1(t+1)^{\perp}} \leq \alpha_{\tau}^{t-\tau} \norm{z_1(\tau + 1)^{\perp}}, \, \forall t > \tau. \label{eqn:z3}
\end{align}
Similarly, from~\eqref{eqn:z1} we have
\begin{align}
    & \norm{z_1(\tau+1)^{\perp}} \leq \alpha_{\tau} \norm{z_1(\tau)^{\perp}} \leq \alpha_{0} \norm{z_1(\tau)^{\perp}}, \nonumber \\
    \implies & \norm{z_1(\tau+1)^{\perp}} \leq \alpha_{0}^{\tau+1} \norm{z(0)^{\perp}}. \label{eqn:z4}
\end{align}
Combining~\eqref{eqn:z3} and~\eqref{eqn:z4},
\begin{align*}
    \norm{z_1(t+1)^{\perp}} & \leq \alpha_{\tau}^{t-\tau} \alpha_{0}^{\tau+1} \norm{z(0)^{\perp}} \\
    & = \left(r_{\tau} \eta \right)^{t-\tau} \alpha_{0}^{\tau+1} \norm{z(0)^{\perp}} \\
    & = \left(r_{\tau} \eta \right)^{(t+1)-(\tau+1)} \alpha_{0}^{\tau+1} \norm{z(0)^{\perp}} \\
    & = \left(r_{\tau} \eta \right)^{(t+1)} \, \underbrace{\left( \dfrac{\alpha_{0}}{r_{\tau} \eta} \right)^{\tau + 1}}_c  \, \norm{z(0)^{\perp}}, \, \forall t > \tau
\end{align*}
which proves the first part of the claim.

Since both $r_{\tau}, \, \eta \in (0,1)$, we have $\underset{t \rightarrow \infty}{\lim} \, \left(r_{\tau} \eta \right)^{(t+1)} = 0$, and the second part of the clam follows from~\eqref{eqn:z2}.

Since $r_{\tau} < 1$, we also have $r_{\tau} \eta < \eta < 1$. Thus, there exists $t_{sw} < \infty$ such that~\eqref{eqn:tsw} holds. To find an explicit form of $t_{sw}$, we want
\begin{align*}
    & c \left(r_{\tau}\eta \right)^{t+1} < \eta^{t+1} \\
    \iff & c \, r_{\tau}^{t+1} < 1 \\
    \iff & \left(\dfrac{1}{r_{\tau}} \right)^{t+1} > \dfrac{1}{c} \\
    \iff & t > \dfrac{log \left(\dfrac{1}{c} \right)}{log \left(\dfrac{1}{r_{\tau}} \right)} - 1.
\end{align*}
Hence, the least such integer $t_{sw}$ is given by $\floor{\dfrac{log \left(\dfrac{1}{c} \right)}{log \left(\dfrac{1}{r_{\tau}} \right)}}$, and the third part of the claim follows.
\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\underline{For $a=1$}, consider Algorithm-I and Algorithm-II in Claim~\ref{thm:clm3} respectively to be Algorithm~\ref{algo_1} and the DGD algorithm. From Theorem~\ref{thm:thm1}, $\alpha_t = \left(\ro+\sigma_0 (\rho^*_K)^{t+1} \right)$. Moreover, $\eta_t = \rho^{(1)} = \rho_{GD} < 1, \, \forall t$. Since $\rho_K^* < 1$, $\{\alpha_t > 0\}_{t \geq 0}$ is strictly decreasing sequence and $\lim_{t \rightarrow \infty}\alpha_t = \ro$. From~\eqref{eqn:conv_dgd} and~\eqref{eqn:rho_def}, $\ro < \eta_t$ if $\beta > 0$ and $\kappa(\A)>1$. 
From Claim~\ref{thm:clm2} it follows that,there exists a positive integer $\tau^{(1)}$ such that $\alpha_t < \eta_t < 1 \, \forall t > \tau^{(1)}$. So, the conditions of Claim~\ref{thm:clm3} hold.

Define, $r_{t} := \dfrac{\alpha_{t}}{\eta_t}$. Then $r_t < 1 \, \forall t>\tau^{(1)}$. Since $\{\alpha_t > 0\}_{t \geq 0}$ is strictly decreasing sequence and $\eta_t$ is a constant, $\{r_t<1\}_{t>\tau^{(1)}}$ is a strictly decreasing sequence. 
So, $\Bar{r} = r_{\tau^{(1)}+1}$.

We have $\tau^{(1)}$ as the least integer satisfying $\alpha_{\tau+1} < \eta$. To get an explicit form of $\tau^{(1)}$:
\begin{align*}
    & \ro+\sigma_0 (\rho^*_K)^{\tau^{(1)}+1} < \rho^{(1)} \\
    \iff & \left(\dfrac{1}{\rho_K^*} \right)^{\tau^{(1)}+1} > \dfrac{\sigma_0}{\rho^{(1)} - \ro} \\
    \iff & \tau^{(1)} > \dfrac{log \left(\dfrac{\sigma_0}{\rho^{(1)} - \ro} \right)}{log \left(\dfrac{1}{\rho_K^*} \right)}-1.
\end{align*}
Noting from~\eqref{eqn:r_a} that $r^{(1)} = r_{\tau^{(1)}+1}$, the statement for $a=1$ follows from Claim~\ref{thm:clm3}. \\

For $a=2$ and $a=3$, we only need to show that $\ro < \rho^{(2)}$ and $\ro < \rho^{(3)}$ respectively hold for $\beta < \sqrt{3\lambda \gamma_r}$ and $\beta < \sqrt{\lambda \gamma_r}$, which is easy to verify. The statements for $a=2$ and $a=3$ then follow from the same argument as above for $a=1$. \\

\underline{For $a=2$} we want,
\begin{align*}
    \ro < \rho^{(2)} & \overset{\eqref{eqn:rho_def},\eqref{eqn:rho_nag}}{\iff} \dfrac{(\lambda - \gamma_r)\beta }{(\lambda + \gamma_r)\beta + 2\lambda \gamma_r} < 1 - \dfrac{2}{\sqrt{3\kappa(\A)+1}} \\
    & \iff \dfrac{\kappa(\A)-1}{\kappa(\A)+1 + 2\dfrac{\lambda}{\beta}} < 1 - \dfrac{2}{\sqrt{3\kappa(\A)+1}}.
\end{align*}
Let, $y^2:= \kappa(\A)$ and $p :=  2\dfrac{\lambda}{\beta}+1$. Then,
\begin{align*}
    \ro < \rho^{(2)} & \iff \dfrac{y^2-1}{y^2+p} + \dfrac{2}{\sqrt{3y^2+1}} -1 < 0 \\
    & \iff 2(y^2+p) < \sqrt{3y^2+1} \, (p+1).
\end{align*}
Let, $p=qy+1$ for some $q>0$. Then,
\begin{align*}
    \ro < \rho^{(2)} & \iff 2(y^2+qy+1) < \sqrt{3y^2+1} \, (qy+2) \\
    & \iff (y^2-1) \left(y(3q^2-4)+4q \right) > 0
\end{align*}
Since $y^2 =\kappa(\A) > 1$, we have
\begin{align*}
    \ro < \rho^{(2)} & \iff y(3q^2-4)+4q > 0.
\end{align*}
From the definitions of $p$ and $q$, we have $ q = \dfrac{2\lambda}{\beta y}$. Then,
\begin{align*}
    \ro < \rho^{(2)} & \iff 4y\left(\dfrac{3\lambda^2}{\beta^2 y^2}-1\right)+4q > 0.
\end{align*}
Now we show that, $\beta < \sqrt{3\lambda \gamma_r}$ satisfies the above condition.
\begin{align*}
    0 < \beta < \sqrt{3\lambda \gamma_r} & \iff \beta^2 < 3\lambda \gamma_r \\
    & \iff 1 < \dfrac{3\lambda \gamma_r}{\beta^2} = \dfrac{3\lambda^2\gamma_r}{\beta^2\lambda} = \dfrac{3\lambda^2}{\beta^2\kappa(\A)} = \dfrac{3\lambda^2}{\beta^2 y^2} \\
    & \implies 4y\left(\dfrac{3\lambda^2}{\beta^2 y^2}-1\right)+4q > 0 \iff \ro < \rho^{(2)},
\end{align*}
which is the desired condition. \\

\underline{For $a=3$}, we want
\begin{align*}
    \ro < \rho^{(3)} & \overset{\eqref{eqn:rho_def},\eqref{eqn:rho_hbm}}{\iff} \dfrac{(\lambda - \gamma_r)\beta }{(\lambda + \gamma_r)\beta + 2\lambda \gamma_r} < \dfrac{\sqrt{\kappa(\A)}-1}{\sqrt{\kappa(\A)}+1} \\
    & \iff \dfrac{\kappa(\A)-1}{\kappa(\A)+1 + 2\dfrac{\lambda}{\beta}} < \dfrac{\sqrt{\kappa(\A)}-1}{\sqrt{\kappa(\A)}+1} \\
    & \iff \left(\sqrt{\kappa(\A)}+1\right)^2 < \kappa(\A)+1 + 2\dfrac{\lambda}{\beta} \\
    & \iff \sqrt{\kappa(\A)} < \dfrac{\lambda}{\beta} \\
    & \iff \beta < \sqrt{\lambda \gamma_r},
\end{align*}
which is the desired condition.\\

